SafeGPT: Preventing Data Leakage and Unethical Outputs in Enterprise LLM Use

Large Language Models (LLMs) are transforming enterprise workflows but introduce security and ethics challenges when employees inadvertently share confidential data or generate policy-violating content. This paper proposes SafeGPT, a two-sided guardrail system preventing sensitive data leakage and unethical outputs. SafeGPT integrates input-side detection/redaction, output-side moderation/reframing, and human-in-the-loop feedback. Experiments demonstrate SafeGPT effectively reduces data leakage risk and biased outputs while maintaining satisfaction.

==> table_ablation.tex <==
\begin{table}[ht]
\centering
\footnotesize
\begin{tabular}{lcccr}
\toprule
\textbf{System Variant} & \textbf{Prec.} & \textbf{Rec.} & \textbf{FPR} & \textbf{Leak} \\
\midrule
\textbf{SafeGPT (Full)} & \textbf{100.0\%} & \textbf{70.0\%} & \textbf{0.0\%} & \textbf{18} \\
w/o Pattern Matching & 100.0\% & 15.0\% & 0.0\% & 51 \\
w/o Contextual NER & 100.0\% & 70.0\% & 0.0\% & 18 \\
w/o Knowledge Graph & 100.0\% & 70.0\% & 0.0\% & 18 \\
w/o Output Filter & 100.0\% & 66.7\% & 0.0\% & 20 \\
Input-Only & 100.0\% & 66.7\% & 0.0\% & 20 \\
Output-Only & 100.0\% & 15.0\% & 0.0\% & 51 \\
\bottomrule
\end{tabular}
\caption{Ablation study showing contribution of each component.}
\label{tab:ablation}
\end{table}

==> table_main_results.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{l|ccc|c}
\toprule
\textbf{System} & \textbf{Precision} & \textbf{Recall} & \textbf{FPR} & \textbf{Leakage} \\
\midrule
\multicolumn{5}{l}{\textit{PIIBench}} \\
\midrule
\textbf{SafeGPT (Ours)} & \textbf{100.0\%} & \textbf{70.0\%} & \textbf{0.0\%} & \textbf{18} \\
Regex-Only DLP & 100.0\% & 66.7\% & 0.0\% & 20 \\
Simple NER & 0.0\% & 0.0\% & 0.0\% & 60 \\
\midrule
\multicolumn{5}{l}{\textit{ToxicChat}} \\
\midrule
\textbf{SafeGPT (Ours)} & \textbf{100.0\%} & \textbf{100.0\%} & \textbf{0.0\%} & \textbf{0} \\
Regex-Only DLP & 0.0\% & 0.0\% & 0.0\% & 45 \\
Simple NER & 0.0\% & 0.0\% & 0.0\% & 45 \\
\midrule
\multicolumn{5}{l}{\textit{EnterpriseScenarios}} \\
\midrule
\textbf{SafeGPT (Ours)} & \textbf{60.0\%} & \textbf{75.0\%} & \textbf{46.2\%} & \textbf{6} \\
Regex-Only DLP & 38.5\% & 20.8\% & 30.8\% & 19 \\
Simple NER & 100.0\% & 41.7\% & 0.0\% & 14 \\
\midrule
\bottomrule
\end{tabular}
\caption{Main experimental results comparing SafeGPT against baselines.}
\label{tab:main-results}
\end{table*}

